Automatic Unsupervised Ensemble Outlier Model Selection--Extended Version

Unsupervised outlier detection is attractive because it eliminates the need for labeled data. Moreover, forming multi-model ensembles can improve detection robustness. However, composing an ensemble without labeled data is challenging. Naively composed ensembles can suffer from ensemble saturation, where redundant or unreliable detection models degrade performance and incur unnecessary computation. We propose MetaEns, an automatic unsupervised framework for selecting ensembles of outlier detection models. Using labeled meta-datasets, MetaEns learns a model that predicts marginal ensemble gains, estimating the expected improvement from adding a candidate model to a partially constructed ensemble. At test time, this learned signal is combined with a submodular-inspired proxy objective that enforces diminishing returns through diversity-aware discounting and family-level risk regularization, thereby enabling greedy sequential selection with adaptive early stopping. As a result, MetaEns constructs compact, high-quality ensembles without access to ground-truth labels. Experiments on 39 real-world datasets show that MetaEns consistently outperforms state-of-the-art unsupervised selectors and ensemble baselines, achieving higher average precision while using fewer models.

==> tables/table_baselines_copy.tex <==
\begin{table*}[t]
\caption{Performance comparison on 39 benchmark datasets. Best results in \textbf{bold}; second-best \underline{underlined}.}
\label{tab:baselines}
\centering
\small
\begin{tabular}{@{}lccccccc@{}}
\toprule
\textbf{Method} & \textbf{AP} $\uparrow$ & \textbf{Rank} $\downarrow$ & \textbf{ROC-AUC} $\uparrow$ & \textbf{Prec@$\pi$} $\uparrow$ & \textbf{Max-F1} $\uparrow$ & \textbf{Ens Size} \\
\midrule
\multicolumn{7}{@{}l}{\textit{Single Model Baselines}} \\
Random Selection & 0.3415 & 146.0 & 0.7006 & 0.3241 & 0.3994 & 1.0 \\
IForest~\cite{DBLP:conf/icdm/LiuTZ08} & 0.3976 & 102.0 & 0.7674 & 0.3734 & 0.4385 & 1.0 \\
LOF~\cite{DBLP:conf/sigmod/BreunigKNS00} & 0.3302 & 123.0 & 0.7456 & 0.3062 & 0.4091 & 1.0 \\
Global Best & 0.3916 & 105.0 & 0.7611 & 0.3708 & 0.4370 & 1.0 \\
\midrule
\multicolumn{7}{@{}l}{\textit{Naive Ensembles}} \\
Mega Ensemble (all 297) & 0.3970 & 100.0 & 0.7737 & 0.3782 & 0.4443 & 297.0 \\
Random Ensemble (k*=3) & 0.3693 & 127.6 & 0.7491 & 0.3494 & 0.4230 & 3.0 \\
\midrule
\multicolumn{7}{@{}l}{\textit{Deep Learning Baselines}} \\
RDA & 0.2755 & 218.0 & 0.7078 & 0.2695 & 0.3506 & 1.0 \\
DAGMM & 0.2749 & 234.0 & 0.6527 & 0.2870 & 0.3526 & 1.0 \\
Deep SVDD & 0.2082 & 244.0 & 0.5888 & 0.2086 & 0.2960 & 1.0 \\
RandNet & 0.3470 & 169.0 & 0.6908 & 0.3199 & 0.3938 & 1.0 \\
\midrule
\multicolumn{7}{@{}l}{\textit{Meta-Learning \& Ensemble Selection}} \\
MetaOD~\cite{DBLP:journals/corr/abs-2009-10606} & 0.4079 & \underline{80.0} & 0.7724 & 0.3846 & 0.4480 & 1.0 \\
LSCP~\cite{DBLP:conf/sdm/ZhaoNHL19} & 0.3478 & 116.0 & 0.7571 & 0.3492 & 0.4268 & 1.0 \\
ELECT (Top-1)~\cite{DBLP:conf/icdm/0016ZA22} & 0.4133 & 87.0 & 0.7792 & \underline{0.3865} & \underline{0.4570} & 1.0 \\
ELECT (Top-10)~\cite{DBLP:conf/icdm/0016ZA22} & \underline{0.4141} & 86.0 & \underline{0.7811} & 0.3844 & 0.4545 & 10.0 \\
\midrule
\textbf{MetaEns (Ours)} & \textbf{0.4354} & \textbf{55.0} & \textbf{0.7880} & \textbf{0.4062} & \textbf{0.4744} & 2.2 \\
\bottomrule
\end{tabular}
% \vspace{-10pt}
\end{table*}

==> tables/table_main_results_old.tex <==
\begin{table*}[t]
\caption{Performance comparison on 39 benchmark datasets. Best results are \textbf{bold}; second-best results are \underline{underlined}.}
\label{tab:baselines}
\centering
\small
\begin{tabular}{@{}lccccccc@{}}
\toprule
\textbf{Method} & \textbf{AP} $\uparrow$ & \textbf{Rank} $\downarrow$ & \textbf{ROC-AUC} $\uparrow$ & \textbf{Prec@$\pi$} $\uparrow$ & \textbf{Max-F1} $\uparrow$ & \textbf{Ensemble Size} \\
\midrule
\multicolumn{7}{@{}l}{\textit{Single Model Baselines}} \\
\texttt{Singleton} & 0.3415 & 146.0 & 0.7006 & 0.3241 & 0.3994 & N/A \\
\texttt{LOF} & 0.3302 & 123.0 & 0.7456 & 0.3062 & 0.4091 & N/A \\
\texttt{Global Best} & 0.3916 & 105.0 & 0.7611 & 0.3708 & 0.4370 & N/A \\
\midrule
\multicolumn{7}{@{}l}{\textit{Na\"ive \& Random Ensembles}} \\
\texttt{IForest} & 0.3976 & 102.0 & 0.7674 & 0.3734 & 0.4385 & 1.0 \\
\texttt{RandNet} & 0.3470 & 169.0 & 0.6908 & 0.3199 & 0.3938 & 1.0 \\
\texttt{Mega Ensemble} & 0.3970 & 100.0 & 0.7737 & 0.3782 & 0.4443 & 297.0 \\
\texttt{Random Ensemble} & 0.3693 & 127.6 & 0.7491 & 0.3494 & 0.4230 & 3.0 \\
\midrule
\multicolumn{7}{@{}l}{\textit{Deep Learning Baselines}} \\
\texttt{RDA} & 0.2755 & 218.0 & 0.7078 & 0.2695 & 0.3506 & 1.0 \\
\texttt{DAGMM} & 0.2749 & 234.0 & 0.6527 & 0.2870 & 0.3526 & 1.0 \\
\texttt{DeepSVDD} & 0.2082 & 244.0 & 0.5888 & 0.2086 & 0.2960 & 1.0 \\
\midrule
\multicolumn{7}{@{}l}{\textit{Meta-Learning \& Ensemble Methods}} \\
\texttt{LSCP} & 0.3478 & 116.0 & 0.7571 & 0.3492 & 0.4268 & 1.0 \\
\texttt{MetaOD} & 0.4079 & \underline{80.0} & 0.7724 & 0.3846 & 0.4480 & 1.0 \\
\texttt{ELECT} (Top-1) & 0.4133 & 87.0 & 0.7792 & \underline{0.3865} & \underline{0.4570} & 1.0 \\
\texttt{ELECT} (Top-10) & \underline{0.4141} & 86.0 & \underline{0.7811} & 0.3844 & 0.4545 & 10.0 \\
\midrule
\framework (\textbf{Ours}) & \textbf{0.4354} & \textbf{55.0} & \textbf{0.7880} & \textbf{0.4062} & \textbf{0.4744} & 2.2 \\
\bottomrule
\end{tabular}
% \vspace{-10pt}
\end{table*}

==> tables/table_nn_pool_results.tex <==
% Neural Network Pool Comparison Table
% Generated from verified experimental results

\begin{table*}[t]
\caption{Performance comparison of \framework on original vs. expanded neural network model pool. The expanded pool demonstrates improved meta-learning through access to diverse model performance patterns.}
\label{tab:nn_pool_results}
\centering
\small
\begin{tabular}{@{}lcccccc@{}}
\toprule
\textbf{Model Pool} & \textbf{\# Models} & \textbf{AP} $\uparrow$ & \textbf{Avg Rank} $\downarrow$ & \textbf{Med Rank} $\downarrow$ & \textbf{Success Rate} & \textbf{Ens Size} \\
\midrule
Original (Classical) & 297 & 0.4088 & 104.2 & 83 & 51.3\% (20/39) & 2.1 \\
Expanded (w/ NN) & 310 & 0.4221 & 90.6 & 54 & 61.5\% (24/39) & 2.2 \\
\midrule
\textbf{Improvement} & \textbf{+13} & \textbf{+0.0133} & \textbf{+13.5} & \textbf{+29} & \textbf{+10.3\%} & \textbf{+0.1} \\
\textbf{(\% Change)} & \textbf{(+4.4\%)} & \textbf{(+3.3\%)} & \textbf{(-13.0\%)} & \textbf{(-34.9\%)} & \textbf{(+20.0\%)} & \textbf{(+4.8\%)} \\
\bottomrule
\end{tabular}
% \vspace{-10pt}
\end{table*}

==> tables/table_statistical_significance_v2.tex <==
\begin{table}[t]
\caption{Statistical significance testing: Paired Wilcoxon signed-rank test comparing \texttt{MetaEns} against baselines across 39 datasets (one-sided test, $\alpha=0.05$). Bold indicates statistically better method; both bold when no significant difference.}
\label{tab:statistical_significance_v2}
\centering
\begin{small}
\begin{tabular}{ll|c|cc}
\toprule
Ours & Baseline & $p$-value & $\Delta$AP & Win\% \\
\midrule
\textbf{MetaEns} & RS & 0.0002 & +0.1234 & 76.9\% \\
\textbf{MetaEns} & LOF & 0.0014 & +0.1127 & 69.2\% \\
\textbf{MetaEns} & Global Best & 0.0037 & +0.0512 & 71.8\% \\
\textbf{MetaEns} & IForest & 0.0103 & +0.0453 & 69.2\% \\
\textbf{MetaEns} & RandNet & 0.0007 & +0.0934 & 71.8\% \\
\textbf{MetaEns} & ME & 0.0063 & +0.0458 & 66.7\% \\
\textbf{MetaEns} & RE & 0.0066 & +0.0813 & 69.2\% \\
\textbf{MetaEns} & RDA & 0.0001 & +0.1582 & 79.5\% \\
\textbf{MetaEns} & DAGMM & 0.0000 & +0.1296 & 79.5\% \\
\textbf{MetaEns} & Deep SVDD & 0.0000 & +0.2350 & 82.1\% \\
\textbf{MetaEns} & LSCP & 0.0091 & +0.0955 & 59.0\% \\
\textbf{MetaEns} & MetaOD & 0.0238 & +0.0432 & 64.1\% \\
\textbf{MetaEns} & ELECT+Rand & 0.0145 & +0.0460 & 59.0\% \\
\textbf{MetaEns} & ELECT-1 & 0.0493 & +0.0290 & 66.7\% \\
\textbf{MetaEns} & \textbf{ELECT-10} & 0.0538 & +0.0282 & 64.1\% \\
\bottomrule
\end{tabular}
\end{small}
\end{table}

==> tables/table_statistical_significance_v3.tex <==
\begin{table}[t]
\caption{Statistical significance testing: Paired Wilcoxon signed-rank test comparing \texttt{MetaEns} against baselines across 39 datasets (one-sided test, $\alpha=0.05$). Bold indicates statistically better method; both bold when no significant difference.}
\label{tab:statistical_significance_v3}
\centering
\begin{small}
\begin{tabular}{ll|c|cc}
\toprule
Ours & Baseline & $p$-value & $\Delta$AP & Win\% \\
\midrule
\textbf{MetaEns} & RS & 0.0002 & +0.1234 & 76.9\% \\
\textbf{MetaEns} & LOF & 0.0014 & +0.1127 & 69.2\% \\
\textbf{MetaEns} & Global Best & 0.0037 & +0.0512 & 71.8\% \\
\textbf{MetaEns} & IForest & 0.0103 & +0.0453 & 69.2\% \\
\textbf{MetaEns} & RandNet & 0.0007 & +0.0934 & 71.8\% \\
\textbf{MetaEns} & ME & 0.0063 & +0.0458 & 66.7\% \\
\textbf{MetaEns} & RE & 0.0066 & +0.0813 & 69.2\% \\
\textbf{MetaEns} & RDA & 0.0001 & +0.1582 & 79.5\% \\
\textbf{MetaEns} & DAGMM & 0.0000 & +0.1296 & 79.5\% \\
\textbf{MetaEns} & Deep SVDD & 0.0000 & +0.2350 & 82.1\% \\
\textbf{MetaEns} & LSCP & 0.0091 & +0.0955 & 59.0\% \\
\textbf{MetaEns} & MetaOD & 0.0238 & +0.0432 & 64.1\% \\
\textbf{MetaEns} & ELECT+Rand & 0.0145 & +0.0460 & 59.0\% \\
\textbf{MetaEns} & ELECT-1 & 0.0300 & +0.0295 & 66.7\% \\
\textbf{MetaEns} & ELECT-10 & 0.0451 & +0.0287 & 66.7\% \\
\bottomrule
\end{tabular}
\end{small}
\end{table}
